On Data-Driven Prescriptive Analytics with Side Information: A Regularized Nadaraya-Watson Approach

We consider generic stochastic optimization problems in the presence of side information which enables a more insightful decision. The side information constitutes observable exogenous covariates that alter the conditional probability distribution of the random problem parameters. A decision maker who adapts her decisions according to the observed side information solves an optimization problem where the objective function is specified by the conditional expectation of the random cost. If the joint probability distribution is unknown, then the conditional expectation can be approximated in a data-driven manner using the Nadaraya-Watson (NW) kernel regression. While the emerging approximation scheme has found successful applications in diverse decision problems under uncertainty, it is largely unknown whether the scheme can provide any reasonable out-of-sample performance guarantees. In this paper, we establish guarantees for the generic problems by leveraging techniques from moderate deviations theory. Our analysis motivates the use of a variance-based regularization scheme which, in general, leads to a non-convex optimization problem. We adopt ideas from distributionally robust optimization to obtain tractable formulations. We present numerical experiments for newsvendor and wind energy commitment problems to highlight the effectiveness of our regularization scheme.

==> PCA-attempts.tex <==

{\color{magenta}
\section{PCA Idea}
In the ideal world, we want to solve
\begin{equation*}
\min_{\bm x\in\mathcal X}\; \EErho[\ell(\bm x,\xit)]:=\EE[\ell(\bm x,\xit)\,|\,\gammat=\bm\gamma].
\end{equation*}
But we apply PCA and NW, and solve
\begin{equation*}
\min_{\bm x\in\mathcal X}\; \hat{\EE}[\ell(\bm x,\xit)\,|\,\tilde{\bm \rho}=\bm\rho].
\end{equation*}
Let $\hat{\bm{x}}$ to be the solution of the above optimization (the PCA and NW one). We want to know
\begin{equation*}
\EErho[\ell(\hat{\bm{x}},\xit)] \leq \EErho[\ell(\bm{x^\star},\xit)] + \textbf{???}
\end{equation*}
Using triangle inequality, we know
\begin{equation*}
\begin{aligned}
\left| \EErho[\ell(\hat{\bm{x}},\xit)] - \EErho[\ell(\bm{x^\star},\xit)] \right| &\leq \left| \EErho[\ell(\hat{\bm{x}},\xit)] - \min_{\bm x\in\mathcal X}\; \hat{\EE}_{\bm\rho}[\ell(\bm x,\xit)] \right|  + \left| \min_{\bm x\in\mathcal X}\; \hat{\EE}_{\bm\rho}[\ell(\bm x,\xit)] - \EErho[\ell(\bm{x^\star},\xit)] \right|   \\
&\leq \left| \EErho[\ell(\hat{\bm{x}},\xit)] - \EE_{\bm\rho}[\ell(\hat{\bm{x}},\xit)] \right| + \left| \EE_{\bm\rho}[\ell(\hat{\bm{x}},\xit)] - \min_{\bm x\in\mathcal X}\; \hat{\EE}_{\bm\rho}[\ell(\bm x,\xit)] \right| \\
& +\left| \min_{\bm x\in\mathcal X}\; \hat{\EE}_{\bm\rho}[\ell(\bm x,\xit)] - \EE_{\bm\rho}[\ell(\bm{x}^\star,\xit)] \right|
+ \left| \EE_{\bm\rho}[\ell(\bm{x}^\star,\xit)] - \EErho[\ell(\bm{x^\star},\xit)] \right|
\end{aligned}
\end{equation*}
No sure if this is the right way of doing this...

\subsection{Try bounding 1 (10-7-2020) -- NW with Gaussian kernel}
We have $\tilde{\rho} = \bm{W}\tilde{\bm{\gamma}}$ (the unknown true $\bm{W}$) and $\tilde{\rho}' = \bm{W}'\tilde{\bm{\gamma}}$ (from PCA). Applying NW with $\bm{W}$ (similarly for $\bm{W}'$), we have
\begin{equation*}
\frac{\sum_{i=1}^n\mathcal K_{h}(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i)\ell(\bm x,\bm\xi^i)}{\sum_{i=1}^n\mathcal K_{h}(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma^i})},
\end{equation*}
where the kernel function $\mathcal K_{h}$ is defined through the multivariate Gaussian density  function. Notice that
\begin{equation*}
\mathcal K_h(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i)=\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i\|_2^2}{2h^2}\right) = \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)
\end{equation*}
(Clint: I am actually not sure if $\bm{W}^\top\bm{W}$ is positive definite   so it might not be a norm...... {\color{blue} $\bm{W}^\top\bm{W}$ is psd since $x^\top\bm{W}^\top\bm{W}x= \lVert \bm{W} x \rVert^2\geq 0$ ? } In what follows, we use the notation
\begin{equation*}
\mathcal K_h^{\bm{W}}(\bm{\gamma}-\bm{\gamma}^i) = \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right).
\end{equation*}
Thus, we want to bound
\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i)\right\vert     \\
=&\displaystyle \left\vert\sum_{i=1}^n \left( \frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}  - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right) \ell(\bm x,\bm\xi^i)\right\vert     \\
\leq &\displaystyle \left( \sum_{i=1}^n \left\vert \ell(\bm x,\bm\xi^i)\right\vert\right) \max_i \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert 
 \\
\leq &\displaystyle n \cdot \max_i \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert 
\end{array}
\end{equation*}
where the first inequality holds because of Cauchy Schwarz inequality (one and infinity norm), and the second inequality holds because $\left\vert \ell(\bm x,\bm\xi^i)\right\vert \leq 1$. Notice that by definition, we have
\begin{equation*}
\begin{array}{rl}
\displaystyle \frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}  &\displaystyle = \;\; \frac{\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)}{\sum_{j=1}^n \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)} \\
     &\displaystyle = \;\; \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right) \right)^{-1}
\end{array}
\end{equation*}
Without loss of generality, assume that the one with $\bm{W}$ is larger. We have
\begin{multline*}
\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} 
\\
=  \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right) \right)^{-1} - \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}\right) \right)^{-1} 
\end{multline*}
To bound the above term, we realize that 
\begin{equation*}
x_1 - x_2 = \exp(\log(x_1)) - \exp(\log(x_2)).
\end{equation*}
Thus, we take the log and 
\begin{equation*}
\begin{array}{rl}
& \displaystyle \log \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right) \right)^{-1}\\
= & \displaystyle - \log \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right) \right)\\
\leq & \displaystyle - \max_j \frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2}
\end{array}
\end{equation*}
where the inequality holds because of LogSumExp. Similarly, we have
\begin{equation*}
\begin{array}{rl}
& \displaystyle \log \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}\right) \right)^{-1} \\
= & \displaystyle - \log \left( \sum_{j=1}^n  \exp\left(\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}\right) \right)\\
\geq & \displaystyle - \max_j \frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2} - \log(n)
\end{array}
\end{equation*}
Combine the two above inequalities, we have 
\begin{equation*}
\begin{array}{rl}
& \displaystyle  \frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \\
\leq &\displaystyle  \exp\left( - \max_j \frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2}{2h^2} \right) - \exp\left(- \max_j \frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2} - \log(n) \right) \\
= &\displaystyle  \exp\left( \min_j \frac{\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}^\top\bm{W}}^2 -\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2} \right) - \frac{1}{n}\exp\left( \min_j \frac{\|\bm{\gamma}-\bm{\gamma}^j\|_{\bm{W}'^\top\bm{W}'}^2 -\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}  \right)
\end{array}
\end{equation*}

\subsection{Try bounding 2 (13-7-2020) -- NW with Gaussian kernel}
We begin with some propositions/lemma

\begin{lemma}
Consider $\{a_i\}_{i=1}^n$ and $\{b_i\}_{i=1}^n$ where $a_i,b_i > 0$ for $i\in[n]$. Then
\begin{equation*}
\sum_i \left\vert \frac{a_i}{\sum_j a_j} - \frac{b_i}{\sum_j b_j}  \right\vert \leq 2 \frac{\sum_j \vert b_j - a_j\vert}{\sum_j a_j}
\end{equation*}
\end{lemma}
\begin{proof}
We know
\begin{equation*}
\begin{array}{rl}
\displaystyle  \frac{a_i}{\sum_j a_j} - \frac{b_i}{\sum_j b_j}  
&=\displaystyle\;\; \frac{a_i (\sum_j b_j) - b_i (\sum_j a_j)}{(\sum_j a_j)(\sum_j b_j)}  
\\
&=\displaystyle \frac{a_i (\sum_j b_j) - b_i (\sum_j b_j) + b_i (\sum_j b_j) - b_i (\sum_j a_j)}{(\sum_j a_j)(\sum_j b_j)}  
\\
&=\displaystyle \frac{(a_i-b_i) (\sum_j b_j) + b_i (\sum_j b_j - a_j)}{(\sum_j a_j)(\sum_j b_j)} 
\end{array}
\end{equation*}
Thus we have
\begin{equation*}
\sum_i \left\vert \frac{a_i}{\sum_j a_j} - \frac{b_i}{\sum_j b_j}  \right\vert = \sum_i \left\vert \frac{(a_i-b_i) (\sum_j b_j) + b_i (\sum_j b_j - a_j)}{(\sum_j a_j)(\sum_j b_j)}   \right\vert.
\end{equation*}
Since $a_i, b_i > 0$,
\begin{equation*}
 \left\vert \frac{(a_i-b_i) (\sum_j b_j) + b_i (\sum_j b_j - a_j)}{(\sum_j a_j)(\sum_j b_j)}   \right\vert \leq \frac{\vert a_i-b_i\vert (\sum_j b_j) + b_i (\sum_j \vert b_j - a_j\vert )}{(\sum_j a_j)(\sum_j b_j)}  .
\end{equation*}
So we have
\begin{equation*}
\sum_i \left\vert \frac{a_i}{\sum_j a_j} - \frac{b_i}{\sum_j b_j}  \right\vert \leq \sum_i \frac{\vert a_i-b_i\vert (\sum_j b_j) + b_i (\sum_j \vert b_j - a_j\vert )}{(\sum_j a_j)(\sum_j b_j)} = 2 \frac{\sum_j \vert b_j - a_j\vert}{\sum_j a_j}.
\end{equation*}
\end{proof}
\begin{proposition}
Consider $a,b \leq 0$, then
\begin{equation*}
\vert \exp(b)-\exp(a) \vert \leq \vert b-a \vert
\end{equation*}
\end{proposition}
\begin{proof}
Without loss of generality, assume $b\geq a$. By mean value theorem, 
\begin{equation*}
\frac{\exp(b)-\exp(a)}{b-a} = \exp(c),
\end{equation*}
where $c\in[a,b]$. Since $a\leq b\leq 0$, $\exp(c) \leq \exp(0) = 1$. Thus, we have
\begin{equation*}
\exp(b)-\exp(a)\leq b-a.
\end{equation*}
\end{proof}
\textbf{We now try to bound the NW terms.} We have $\tilde{\rho} = \bm{W}\tilde{\bm{\gamma}}$ (the unknown true $\bm{W}$) and $\tilde{\rho}' = \bm{W}'\tilde{\bm{\gamma}}$ (from PCA). Applying NW with $\bm{W}$ (similarly for $\bm{W}'$), we have
\begin{equation*}
\frac{\sum_{i=1}^n\mathcal K_{h}(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i)\ell(\bm x,\bm\xi^i)}{\sum_{i=1}^n\mathcal K_{h}(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma^i})},
\end{equation*}
where the kernel function $\mathcal K_{h}$ is defined through the multivariate Gaussian density  function. Notice that
\begin{equation*}
\mathcal K_h(\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i)=\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{W}\bm{\gamma}-\bm{W}\bm{\gamma}^i\|_2^2}{2h^2}\right) = \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)
\end{equation*}
(Clint: I am actually not sure if $\bm{W}^\top\bm{W}$ is positive definite   so it might not be a norm...... {\color{blue} $\bm{W}^\top\bm{W}$ is psd since $x^\top\bm{W}^\top\bm{W}x= \lVert \bm{W} x \rVert^2\geq 0$ ? } In what follows, we use the notation
\begin{equation*}
\mathcal K_h^{\bm{W}}(\bm{\gamma}-\bm{\gamma}^i) = \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right).
\end{equation*}
Thus, we want to bound
\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i)\right\vert     \\
=&\displaystyle \left\vert\sum_{i=1}^n \left( \frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}  - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right) \ell(\bm x,\bm\xi^i)\right\vert     \\
\leq &\displaystyle \left( \max_i \left\vert \ell(\bm x,\bm\xi^i)\right\vert\right)  \sum_{i=1}^n\left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert 
 \\
\leq &\displaystyle \sum_{i=1}^n \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert 
\end{array}
\end{equation*}
where the first inequality holds because of Cauchy Schwarz inequality (one and infinity norm), and the second inequality holds because $\left\vert \ell(\bm x,\bm\xi^i)\right\vert \leq 1$. Using the Lemma above, we have
\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i)\right\vert     \\
\leq &\displaystyle \sum_{i=1}^n \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert  \\
\leq &\displaystyle 2 \frac{\sum_{i=1}^n \left\vert  \mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i) - \mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)\right\vert}{\sum_{j=1}^n \mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^j)}.
\end{array}
\end{equation*}
Notice that using our above proposition, we have
\begin{equation*}
\begin{array}{rl}
\displaystyle \left\vert  \mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i) - \mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)\right\vert 
&=\displaystyle\;\; \left\vert \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}\right) - \frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)\right\vert  \\
&=\displaystyle\;\; \frac{1}{{(2\pi)}^{d/2}} \left\vert  \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2}\right) -  \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)\right\vert  \\
&\leq\displaystyle\;\; \frac{1}{{(2\pi)}^{d/2}} \left\vert  \frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 - \|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2}{2h^2} \right\vert  \\
\end{array}
\end{equation*}
Thus, we have
\begin{multline*}
\left\vert\sum_{i=1}^n\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i)\right\vert \\
\leq 2 \dfrac{\sum_{i=1}^n \Big\vert \|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2 - \|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}'^\top\bm{W}'}^2 \Big\vert}{2h^2 \sum_{j=1}^n \mathcal  \exp\left(-\frac{\|\bm{\gamma}-\bm{\gamma}^i\|_{\bm{W}^\top\bm{W}}^2}{2h^2}\right)}
\end{multline*}

Note that when $\bm{W} = \bm{W}'$, the right hand side is $0$.
}


{\color{blue}
\noindent Possible Approach
\begin{itemize}
    \item Assume $\gamma\in \mb R^D$ in a low-dimensional subspace with dimensionality $d \ll D$, i.e., there exist $W\in \mb R^{d\times D}$ and $v\in \mb R^d$ such that $\rho = W\gamma+v$.
    \item To keep points independent of each other for application of moderate/large deviation theory, split the original dataset into two parts - $P_1$ of size $n_1=n/\log n$ and $P_2$ of size $n-n_1$. Use points in $P_1$ to estimate $\hat{W}$ and $\hat{v}$
    \item Assuming a sub-gaussian probability distribution, show that $\lVert\Sigma-\hat{\Sigma}\rVert_{\fr}\leq \sqrt{\frac{D \log n}{n}}$ with probability at least $1-\tilde{O}(n^{-D})$.
    \item Use Davis-Kahan to obtain a bound on $\lVert W- \hat{W}O\rVert_{\fr}\leq \frac{1}{\lambda_d}\lVert\Sigma-\hat{\Sigma}\rVert_{\fr} \lesssim \frac{1}{\lambda_d} \sqrt{\frac{D \log n}{n}}$. Also note $\lVert v-\hat{v}\lVert\lesssim \frac{1}{\sqrt{n}}$. Then 
    \begin{equation*}
    \begin{aligned}
            \lVert \rho-\hat{\rho} \rVert_2 &= \lVert (W-\hat{W})\gamma + (v-\hat{v})\rVert_2\\
            &\leq \| (W-\hat{W})\|_2 \|\gamma\|_2+   \|v-\hat{v}\|_2\\
            &\leq \| (W-\hat{W})\|_{\fr} \|\gamma\|_2+   \|v-\hat{v}\|_2 \\
            &\lesssim \frac{1}{\lambda_d} \sqrt{\frac{D \log n}{n}} \lVert \gamma \rVert_2+ \frac{1}{\sqrt{n}} 
    \end{aligned}
    \end{equation*}
    \item Some assumption on the kernel function 
\end{itemize}
\begin{equation*}
\mathcal K_h(\bm{x})=\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{\|\bm {x}\|_2^2}{2h^2}\right) = C \exp\left(-\frac{\|\bm {x}\|_2^2}{2h^2}\right)
\end{equation*}
Next, we compute $\nabla_x \mathcal K_h$. We note that 
\begin{equation*}
    \nabla_x\mathcal K_h= C \exp\left(-\frac{\|\bm {x}\|_2^2}{2h^2}\right) \cdot -\frac{\bm{x}}{h^2}
\end{equation*}
Therefore, we have 
\begin{equation*}
    \| \nabla_x\mathcal K_h \|= \frac{C}{h} \exp\left(-\frac{\|\bm {x}\|_2^2}{2h^2}\right) \cdot \frac{\bm{\| x\|}}{h} \leq \frac{C'}{h}.
\end{equation*}
Thus, $L=\frac{C'}{h}$ is the Lipschitz constant, which implies 
$\|\mathcal K_h(\bm{x}) - \mathcal K_h(\bm{x}')\|\leq \frac{C'}{h} \|\bm{x}-\bm{x}' \|  $. Next, we want to bound  

\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \ell(\bm x,\bm\xi^i)\right\vert     \\
=&\displaystyle \left\vert\sum_{i=1}^n \left( \frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}  - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right) \ell(\bm x,\bm\xi^i)\right\vert     \\
\leq &\displaystyle \left( \max_i \left\vert \ell(\bm x,\bm\xi^i)\right\vert\right) \sum_{i=1}^n \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert 
 \\
\leq &\displaystyle \sum_{i=1}^n \left\vert\frac{\mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})} - \frac{\mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i)}{\sum_{j=1}^n\mathcal K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma^j})} \right\vert \\
\leq &\displaystyle \frac{2\sum_{i=1}^n \left\vert \mathcal  K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma}^i) - \mathcal  K^{\bm{W}'}_{h}(\bm{\gamma}-\bm{\gamma}^i) \right\vert}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}\\
\leq & \displaystyle \frac{2L \sum_{i=1}^n \| \bm{W}(\bm{\gamma}-\bm{\gamma}^i)-\bm{W'}(\bm{\gamma}-\bm{\gamma}^i)\|}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}\\
\leq & \displaystyle \frac{2L \sum_{i=1}^n \| \bm{W}(\bm{\gamma}-\bm{\gamma}^i)-\bm{W'}(\bm{\gamma}-\bm{\gamma}^i)\|}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}\\
\leq & \displaystyle \frac{2L \|\bm{W}-\bm{W'}\| \sum_{i=1}^n \|\bm{\gamma}-\bm{\gamma}^i)\|}{\sum_{j=1}^n\mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}\\
\leq & \displaystyle 2L \|\bm{W}-\bm{W'}\| \cdot \frac {n \max_i \|\bm{\gamma}-\bm{\gamma}^i\|}{n \min_j \mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}\\
= & \displaystyle 2L \|\bm{W}-\bm{W'}\| \cdot \frac {\max_i \|\bm{\gamma}-\bm{\gamma}^i\|}{ \min_j \mathcal K^{\bm{W}}_{h}(\bm{\gamma}-\bm{\gamma^j})}
\end{array}
\end{equation*}}

\section{Proof for Laplace Kernel}
\noindent Possible Approach
\begin{itemize}
    \item Assume $\gamma\in \mb R^D$ is drawn from a sub-gaussian probability distribution with sub-gaussian parameter $\sigma^2$. Furthermore, we assume that $\gamma$ lies in a low-dimensional subspace with dimensionality $d \ll D$, i.e., there exist $W\in \mb R^{d\times D}$ and $v\in \mb R^d$ such that $\rho = W\gamma+v$.
    \item To keep points independent of each other for application of moderate/large deviation theory, split the original dataset into two parts - $P_1$ of size $n_1=n/\log n$ and $P_2$ of size $n-n_1$. Use points in $P_1$ to estimate $\hat{W}$ and $\hat{v}$
    \item Under the assumption of a sub-gaussian probability distribution, show that $\lVert\Sigma-\hat{\Sigma}\rVert_{\fr}\leq \sqrt{\frac{D \log n}{n}}$ with probability at least $1-\tilde{O}(n^{-D})$.
    \item Use Davis-Kahan to obtain a bound on $\lVert W- \hat{W}O\rVert_{\fr}\leq \frac{1}{\lambda_d}\lVert\Sigma-\hat{\Sigma}\rVert_{\fr} \lesssim \frac{1}{\lambda_d} \sqrt{\frac{D \log n}{n}}$. Also note $\lVert v-\hat{v}\lVert\lesssim \frac{1}{\sqrt{n}}$. Then 
\end{itemize}

\begin{equation}
\label{eq:rho_bound}
\begin{aligned}
        \lVert \bm\rho-\hat{\bm\rho} \rVert_2 &= \lVert (\bm W-\hat{\bm W})\bm\gamma + (\bm v-\hat{\bm v})\rVert_2\\
        &\leq \| (\bm W-\hat{\bm W})\|_2 \|\bm \gamma\|_2+   \|\bm v-\hat{\bm v}\|_2\\
        &\leq \| (\bm W-\hat{\bm W})\|_{\fr} \|\bm \gamma\|_2+   \|\bm v-\hat{\bm v}\|_2 \\
        &\lesssim \frac{1}{\lambda_d} \sqrt{\frac{D \log n}{n}} \lVert \gamma \rVert_2+ \frac{1}{\sqrt{n}} 
\end{aligned}
\end{equation}
Next, we use the result from the following lemma: 
\begin{itemize}
    \item \textbf{Lemma:} Let $\bm X\in SG_d(\sigma^2)$,$\|\bm X \|=\sqrt{\sum_{i=1}^d X_i^2}$, then with probability $1-\delta$ for $\delta\in(0,1)$
    \begin{equation*}
        \| \bm X \| \leq 4\sigma\sqrt{d}+2\sigma\sqrt{\log\bigg(\frac{1}{\delta}\bigg)}
    \end{equation*}
\end{itemize}
We define $\gm_{\max}:=4\sigma(\sqrt{d}+\sqrt{\log n})$. Thus, $\|\bm \gamma\|\leq \gm_{\max}$ with probability atleast $1-\frac{1}{n^2}$.\\

\noindent We define the Laplace kernel as follows:
\begin{equation*}
\mathcal K_h(x)=\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{x}{h}\right)
\end{equation*}
For any generic $\gm \in \mb R^{D}$, we define its projection in the low-dimensional space as $\bm\rho=\bm W \bm\gm \in \mb R^{d}$. Similarly, each $\bm\gm_i \in \mb R^{D}$ is expressed as $\bm\rho_i=\bm W \bm\gm_i \in \mb R^{d}$. Since the true subspace is not known, we estimate the projection matrix by $\hat{\bm W}$ obtained using PCA, and denote the estimated projections of $\bm\rho$ and $\bm \rho_i$  by $\bm\rho'$ and $\bm \rho_i'$ respectively. Let $\eta_i=\|\bm\rho-\bm\rho_i\|$ and $\eta_i'=\|\bm\rho'-\bm\rho_i'\|$. From \eqref{eq:rho_bound}, we first note that $\|\bm\rho-\bm\rho'\|\leq \tau$ and $\|\bm\rho_i-\bm\rho_i'\|\leq \tau$. Therefore, by using reverse triangle and triangle inequalities, we get $|\eta_i-\eta_i'|\leq \| (\bm\rho-\bm\rho_i)- (\bm\rho'-\bm\rho'_i)\| \leq \| \bm\rho-\bm\rho_i\|+\| \bm\rho'-\bm\rho'_i\|  \leq 2\tau$.
\begin{equation}
\label{eq:PCA_bound}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \ell(\bm x,\bm\xi^i)\right\vert\\
\leq &\displaystyle \left( \max_i \left\vert \ell(\bm x,\bm\xi^i)\right\vert\right) \sum_{i=1}^n\left\vert\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} - \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \right\vert\\
\leq &\displaystyle\sum_{i=1}^n\left\vert\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} - \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \right\vert 
\end{array}
\end{equation}
Next, we note that 
\begin{equation*}
\begin{aligned}
    &\displaystyle\left\vert\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} - \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \right\vert \\
    =&\max\bigg\{ \frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)}- \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')},  \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')}- \frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \bigg\} \\
    \leq &\max\bigg\{ \frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)}- \frac{\mathcal  K_{h}(\eta_i+2\tau)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j-2\tau)},  \frac{\mathcal  K_{h}(\eta_i-2\tau)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j+2\tau)}- \frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \bigg\} \\ 
    = &\displaystyle\max\bigg\{ \frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)}- \frac{\exp(-(\eta_i+2\tau)/h)}{\sum_{j=1}^n\exp(-(\eta_j-2\tau)/h)},  \frac{\exp(-(\eta_i-2\tau)/h)}{\sum_{j=1}^n \exp(-(\eta_j+2\tau)/h)}- \frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)} \bigg\} \\ 
    = &\frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)} \max\big\{1-\exp(-4\tau/h), (\exp(4\tau/h)-1) \big\}\\
    \leq &\frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)} (\exp(4\tau/h)-1) 
\end{aligned}
\end{equation*}
Here, we obtain the last equality by considering each of the two terms within the max separately. We first evaluate the first term
\begin{equation*}
    \begin{aligned}
         &\frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)}- \frac{\exp(-(\eta_i+2\tau)/h)}{\sum_{j=1}^n\exp(-(\eta_j-2\tau)/h)}\\
        =&\frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)} (1-\exp(-4\tau/h))
    \end{aligned}
\end{equation*}
Next, we consider the second term
\begin{equation*}
    \begin{aligned}
        &\frac{\exp(-(\eta_i-2\tau)/h)}{\sum_{j=1}^n \exp(-(\eta_j+2\tau)/h)}- \frac{\exp(-\eta_i/h)}{\sum_{j=1}^n\mathcal\exp(-\eta_j/h)}\\
        = & \frac{\exp(-\eta_i)}{\sum_{j=1}^n \exp(-\eta_j)}  (\exp(4\tau/h)-1)
    \end{aligned}
\end{equation*}
Therefore, from \eqref{eq:PCA_bound} we get 
\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \ell(\bm x,\bm\xi^i)\right\vert\leq \exp(4\tau/h)-1.
\end{array}
\end{equation*}

\subsection{Attempt to extend the same idea to gaussian kernel}

\noindent We define the Gaussian kernel as follows:
\begin{equation*}
\mathcal K_h(x)=\frac{1}{{(2\pi)}^{d/2}} \exp\left(-\frac{ {x}^2}{h^2}\right)
\end{equation*}
For any generic $\gm \in \mb R^{D}$, we define its projection in the low-dimensional space as $\bm\rho=\bm W \bm\gm \in \mb R^{d}$. Similarly, each $\bm\gm_i \in \mb R^{D}$ is expressed as $\bm\rho_i=\bm W \bm\gm_i \in \mb R^{d}$. Since the true subspace is not known, we estimate the projection matrix by $\hat{\bm W}$ obtained using PCA, and denote the estimated projections of $\bm\rho$ and $\bm \rho_i$  by $\bm\rho'$ and $\bm \rho_i'$ respectively. Let $\eta_i=\|\bm\rho-\bm\rho_i\|$ and $\eta_i'=\|\bm\rho'-\bm\rho_i'\|$. From \eqref{eq:rho_bound}, we first note that $\|\bm\rho-\bm\rho'\|\leq \tau$ and $\|\bm\rho_i-\bm\rho_i'\|\leq \tau$. Therefore, by using reverse triangle and triangle inequalities, we get $|\eta_i-\eta_i'|\leq \| (\bm\rho-\bm\rho_i)- (\bm\rho'-\bm\rho'_i)\| \leq \| \bm\rho-\bm\rho_i\|+\| \bm\rho'-\bm\rho'_i\|  \leq 2\tau$. Next, we obtain a lower-bound on $\eta_i'^2$. Using the fact that $(\eta_i-\eta_i')^2 \geq 0$, we note that
\begin{equation*}
\begin{aligned}
    \eta_i'^2&\geq -\eta_i^2 + 2\eta_i \eta_i' \\
    &\geq -\eta_i^2 + 2\eta_i (\eta_i -2\tau) \\
    &= \eta_i^2- 4\eta_i \tau  \\
    &\geq \eta_i^2- 8\gm_{\max}\tau 
\end{aligned}
\end{equation*}
We want to bound the following quantity
\begin{equation}
\label{eq:PCA_bound2}
\begin{aligned}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \ell(\bm x,\bm\xi^i)\right\vert\\
\leq &\displaystyle \left( \max_i \left\vert \ell(\bm x,\bm\xi^i)\right\vert\right) \sum_{i=1}^n\left\vert\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} - \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \right\vert\\
    \leq&\displaystyle\sum_{i=1}^n\left\vert\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} - \frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \right\vert \\
    \leq&\displaystyle \frac{2}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)}\sum_{i=1}^n|\mathcal  K_{h}(\eta_i) - \mathcal  K_{h}(\eta_i')|
\end{aligned}
\end{equation}
{\color{blue} (Clint: why the above holds?)(Prateek: Using your lemma?) } Next, we consider
\begin{equation*}
    \begin{aligned}
        &|\mathcal  K_{h}(\eta_i) - \mathcal  K_{h}(\eta_i')| \\
        =&\max\big\{ K_{h}(\eta_i) - \mathcal  K_{h}(\eta_i'), K_{h}(\eta_i') - \mathcal  K_{h}(\eta_i) \big\}\\
        \leq & C\max\bigg\{ \exp\bigg(-\frac{\eta_i^2}{h^2}\bigg)-\exp\bigg(-\frac{(\eta_i+2\tau)^2}{h^2}\bigg), \exp\bigg(-\frac{(\eta_i^2-8\gamma_{\max}\tau)}{h^2}\bigg)- \exp\bigg(-\frac{\eta_i^2}{h^2}\bigg) \bigg\} \\
        \leq & C \exp\bigg(-\frac{\eta_i^2}{h^2}\bigg) \max\bigg\{ 1-\exp\bigg(-\frac{(8\gamma_{\max}\tau+4\tau^2)}{h^2}\bigg) ,\exp\bigg(\frac{8\gamma_{\max}\tau}{h^2}\bigg)-1\bigg) \bigg\}\\
        \leq & C \exp\bigg(-\frac{\eta_i^2}{h^2}\bigg) \max\bigg\{ 1-\exp\bigg(-\frac{(8\gamma_{\max}\tau+4\tau^2)}{h^2}\bigg) ,\exp\bigg(\frac{8\gamma_{\max}\tau+4\tau^2}{h^2}\bigg)-1\bigg) \bigg\}\\
        \leq & C \exp\bigg(-\frac{\eta_i^2}{h^2}\bigg)\bigg( \exp\bigg(\frac{8\gamma_{\max}\tau+4\tau^2}{h^2}\bigg)-1\bigg)\\
\end{aligned}
\end{equation*}


\noindent Here, we obtain the last equality by considering each of the two terms within the max separately. We first evaluate the first term
\begin{equation*}
\begin{aligned}
        &\exp\bigg(-\frac{\eta_i^2}{h^2}\bigg)-\exp\bigg(-\frac{(\eta_i+2\tau)^2}{h^2}\bigg)\\
    \leq &\exp\bigg(-\frac{\eta_i^2}{h^2}\bigg)\bigg(1-\exp\bigg(-\frac{(4\eta_i\tau+4\tau^2)}{h^2}\bigg)\bigg) \\
    \leq &\exp\bigg(-\frac{\eta_i^2}{h^2}\bigg)\bigg(1-\exp\bigg(-\frac{(8\gamma_{\max}\tau+4\tau^2)}{h^2}\bigg)\bigg)
\end{aligned}
\end{equation*}
Therefore, from \eqref{eq:PCA_bound2} we get 
\begin{equation*}
\begin{array}{rl}
&\displaystyle \left\vert\sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i)}{\sum_{j=1}^n\mathcal K_{h}(\eta_j)} \ell(\bm x,\bm\xi^i) - \sum_{i=1}^n\frac{\mathcal  K_{h}(\eta_i')}{\sum_{j=1}^n\mathcal K_{h}(\eta_j')} \ell(\bm x,\bm\xi^i)\right\vert\leq 2 \bigg( \exp\bigg(\frac{8\gamma_{\max}\tau+4\tau^2}{h^2}\bigg)-1\bigg).
\end{array}
\end{equation*}

